Staged Specification Logic for Verifying Higher-Order Imperative Programs (Technical Report)

Higher-order functions and imperative states are language features supported by many mainstream languages. Their combination is expressive and useful, but complicates specification and reasoning, due to the use of yet-to-be-instantiated function parameters. One inherent limitation of existing specification mechanisms is its reliance on only two stages: an initial stage to denote the precondition at the start of the method and a final stage to capture the postcondition. Such two-stage specifications force abstract properties to be imposed on unknown function parameters, leading to less precise specifications for higher-order methods. To overcome this limitation, we introduce a novel extension to Hoare logic that supports multiple stages for a call-by-value higher-order language with ML-like local references. Multiple stages allow the behavior of unknown function-type parameters to be captured abstractly as uninterpreted relations; and can also model the repetitive behavior of each recursion as a separate stage. In this paper, we define our staged logic with its semantics, prove its soundness and develop a new automated higher-order verifier, called Heifer, for a core ML-like language.

==> case-exc.tex <==
\subsubsection{Exceptions}
\label{sec:exceptions}

\begin{figure}
  \begin{subfigure}[b]{.52\linewidth}
\begin{lstlisting}[name=exceptionfailing,numbers=none]
let failing x
  (*@\maybeinferred{$\neffectcall{failing(x,res)} =  \stageexi{i}\stagereq{\heapto{x}{i}}\seq\stageens{\heapto{x}{i{+}1}\wedge i{+}1{=}3}\seq\stageho{E}{}$} @*)
(*@\maybeinferredd{$\vee\ \stageexi{i}\stagereq{\heapto{x}{i}}\seq\stageens{\heapto{x}{i{+}1}\wedge\res{=}i{+}1\wedge i{+}1{\neq}3}$} @*)
= x := !x + 1;
  if x = 3 then raise E else !x
\end{lstlisting}
  \end{subfigure}
  \begin{subfigure}[b]{.45\linewidth}
\begin{lstlisting}[name=exceptionmain,numbers=none]
exception E
let main ()
(*@\maybeinferred{$\neffectcall{main(res)} =\stageexi{y}\stageens{\heapto{y}{3} \wedge \res{=}1}$} @*)
= let y = ref 2 in
  try failing y with E -> 1
\end{lstlisting}
  \end{subfigure}
  \caption{An Example with Exception in Staged Logic}
  \label{fig:exception_example}
  \Description{Exception example}
\end{figure}

\cref{fig:exception_example} demonstrates precise reasoning about exceptional behavior using stages.
If we model an exception as a new kind of stage, the specification for \ml{failing} shows clearly that it has two paths, one of which ends in an exception, and \emph{both} of which have observable side effects on the reference \ml{x}.
We can therefore prove automatically (in \ml{main}) that \ml{failing} violates \emph{strong exception safety}~\cite{Gherghina2010ASL}, as it does not fail transactionally.
We do not present the semantics of \ml{try} formally in this paper but support it in our prototype.


==> completeness.tex <==
\begin{verbatim}
Hyper Hoare Logic
 C ::= skip | x:=e | x:=* | assume b | C1; C2 | C+C | C*

Staged Hoare Logic:
 e ::   c
      | ref x | x:=x2 | !x 
      | let x=e1 in e2 
      | \x* -> e 
      | x(x*)
      | if x then e1 else e2
	  
Need fix point? Need Exist rule?
	  
Soundness
    |- {S1} e {S2}  implies |= {S1} e {S2}
Completeness
    |= {S1} e {S2}  implies |- {S1} e {S2}

Soundness of Forward Rules
  |- {N} e {D} implies |= {N} e {D}

  |= {N} e {D} <->
     forall S0,h0 [S0,h0]->[S,h,Norm(_)] |= N
     ...

Completeness of Forward Rules

Given e,h,S -> h1,S1 /\ S,h,{} |= D -> S2,h2,L /\ S1<:S2
implies {emp} e {D}.


\end{verbatim}


==> compose.tex <==

To better understand why staged specification is a more
comprehensive
mechanism for modelling higher-order programs, let us compare
it with the pre/post Hoare-style specification mechanism that
has traditionally been applied to %
higher-order programs for both imperative \cite{DBLP:journals/jfp/NanevskiMB08,DBLP:conf/icfp/Chargueraud11,DBLP:journals/corr/abs-2011-14044} and
functional languages \cite{DanaXu:POPL09}.


Change to just foldr example..
though applyN is referred in Sec 6 + case study


\begin{verbatim}
```
 rec foldr(f a l) = match l with
     inj1  x1 ⇒ a
   | inj2 x2 ⇒ let h = π1 ! x2 in
            let t = π2 ! x2 in
            f (h ,(foldr f a t))
```

A typical specification for foldr in Iris is:

```
{(∀x. ∀a'. ∀ys. {P x ∗ Inv ys a'} f (x, a') {r.Inv (x:ys) r})
  * isList l xs * all P xs * Inv [] a }
        foldr f a l
{r. isList l xs * Inv xs r}
```

This specification requires two unknowns `P x` and `Inv ys a`
to be provided by proof engineers for every callee of foldr.

In contrast, the \heifer~staged specification for foldr (given App A) is:

```
  foldr$(f,a,l,res) =
        ens l=[] /\ res=a
     \/ ex r',l'. ens l=x:l'; foldr$(f,a,l',r'); f$(x,r',res)
```

One major question that all the reviewers expressed was how our approach
compares with state-of-the-art approaches, such as Iris, for verifying
higher-order imperative programs. We would like to use
foldr as an example to make a clearer comparison here:

```
 rec foldr(f a l) = match l with
     inj1  x1 ⇒ a
   | inj2 x2 ⇒ let h = π1 ! x2 in
            let t = π2 ! x2 in
            f (h ,(foldr f a t))
```

A typical specification for foldr in Iris is:

```
{(∀x. ∀a'. ∀ys. {P x ∗ Inv ys a'} f (x, a') {r.Inv (x:ys) r})
  * isList l xs * all P xs * Inv [] a }
        foldr f a l
{r. isList l xs * Inv xs r}
```

This specification requires two unknowns `P x` and `Inv ys a`
to be provided by proof engineers for every callee of foldr.

In contrast, the \heifer~staged specification for foldr (given App A) is:

```
  foldr$(f,a,l,res) =
        ens l=[] /\ res=a
     \/ ex r',l'. ens l=x:l'; foldr$(f,a,l',r'); f$(x,r',res)
```

The key differences between the two approaches are:

(i)  Simpler use of unknown relation, e.g., `f$`, to capture the specification
     for each yet-to-be instantiated function parameter.

(ii)  Direct use of recursive relation, e.g., `foldr$(..)`, inside
      staged specification of recursive method with function-typed
      parameters.

(iii) Use of staged operator `;` between any two staged specifications,
      where needed. Such staged operator(s) must be utilized either
      before and/or after each unknown/recursive staged relation.

These new features are present in \heifer~(but not in Iris) and
have substantive advantages, as itemized below.

(i) is important since its use allows arbitrary specification
 to be instantiated for each unknown function-type parameter f.
 In contrast, Iris requires a nested Hoare triple
      `{P x ∗ Inv ys a'} f (x, a') {r.Inv (x:ys) r})`,
 where there is an implicit assumption that f(x,a') will return
 normally _without_ any exception or algebraic effect due
 to the presence of `Inv (x:ys)` in its post-state.

 Hence, the above Iris spec for foldr _cannot_ handle f calls that
 may invoke exceptions, such as

```
   f1(x,a)  = if x=0 then raise Exception(a)
              else if x>0 then x+a
              else a
```

  We did mention this capability in our introduction (pg 3),
  but chose originally not to elaborate on this difference.
  Kindly allow us to elaborate on this material difference here.
  (NB: we are aware of an extension to Iris that can handle
    algebraic effects but this extension requires Iris' wp predicate to be parameterized with a new notion of protocols; in contrast,
    exceptions (and algebraic effects) are directly
    supported in staged specifications.)

In particular, \heifer~supports each exception raised as
an uninterpreted relation that may be caught by exception handlers.

In this case, we simply need to instantiate `f$(x,a,res)` with:

```
 f1$(x,a,res) = req x=0; Exception(a)
                \/ req x>0; ens res=x+a
                \/ req x<0; ens res=a
```

where Exception(a) is an uninterpreted relation.

(ii) is important as it allows us to write specification of
recursive higher-order functions _without_ forcing us to design
inductive invariants and pre-conditions upfront, such as `Inv ys a`
and `all P xs`. Any such requirement is implicitly
captured within our recursive staged specification.

(iii) is needed since `;` operator is used to support (i) and (ii).

Though \heifer's approach does not require inductive invariants
and preconditions to be designed upfront, we do require
re-summarization on each instantiated call of recursive
methods (such as foldr) with higher-order parameters to be done
by either proof engineers or a fixed-point calculator. In the
case of `foldr$(f1$,a,l,res)`, one good re-summarization
is as follows:

```
foldr_with_f1$(a,l,res) =
         req nozero(l); ens sumpos(l,a,res)
         \/ req ~nozero(l); Exception(_)
  // pure recursive predicates
  nozero(l) = l=[] \/ (l=x:l'/\x!=0 /\ nozero(l'))
  sumpos(l,a,res) = l=[]/\res=a 
       \/ l=x:l' /\ x>0 /\ sumpos(l',x+a,res)
       \/ l=x:l' /\ x<0 /\ sumpos(l',a,res)
```

In the above, the value `_` captured in the raised exception
is currently lost via over-approximation. To improve this
situation, we can provide a stronger summarization with
the help of another pure `aux` predicate,as follows:

```
 ff2$(a,l,res) = req nozero(l); ens sumpos(l,a,res)
                 req ~nozero(l); ex r; aux(l,a,r) ; Exception(r)
 // where aux is a pure predicate
 aux(l,a,r) = l=[]/\r=a 
     \/ l=x:l' /\ x=0 /\ nozero(l') /\ sumpos(l',a,r)
     \/ l=x:l' /\ x=0 /\ ~nozero(l') /\ aux(l',a,r)
     \/ l=x:l' /\ x!=0 /\ aux(l',a,res))
```

While it may be debatable whether writing an inductive invariant
or providing a re-summarization of a staged specification
is better, we have provided maximum flexibility via \heifer's approach
without any pre-conceived form on the specification of
unknown function-type parameters.

\end{verbatim}



Let us illustrate %
key differences via
a simple higher-order method to compose two functions
together:

\begin{tabbing}
\quad \quad \= \quad \= \coden{let~r2~} \= \kill
\> \coden{\btt{compose}(f,g,x) =} \coden{let~r~{=}~g(x)~in~f(r)}
\end{tabbing}

Here, \coden{f} and \coden{g}, are unspecified function-type
parameters with the result \coden{r}
from \coden{g(x)} call being passed as input into
the \coden{f(r)} call.
Using staged specifications,
we can model each function \coden{mn(x_1,\ldots,x_n)} by its corresponding staged
specification \coden{mn\$(x_1,\ldots,x_n,y)} in relational form with an
extra parameter \coden{y} for denoting the result of its call invocation.
Thus:

\begin{tabbing}
\quad \quad \= \quad \= \coden{let~r2~} \= \kill
\> \coden{compose\$(f,g,x,res) =} \coden{\exists r \,{\cdot}\, g\$(x,r)~{;}~f\$(r,res)}
\end{tabbing}

The above two-stage specification merely states that
there are two (higher-order) function
invocations \coden{g\$(x,r)} and \coden{f\$(r,res)} that are
being executed in sequence, as appropriately separated
by a \coden{;}\, operator.
An existential variable \coden{r} was also used to
capture a value named in the \coden{let} construct;
so as to link the output of \coden{g\$(x,r)} to the
input of \coden{f\$(r,res)}. Such a specification
could not have been more concisely written.

Compare this to the methodology of Hoare-style pre/post specification.
A traditional way of doing this would involve
the following pre/post specification instead:
  
\begin{tabbing}
\quad \quad \= \quad \= \coden{let~r2~} \= \kill
\> \coden{compose\$(f,g,x,res) =} \\
\> \> \coden{\req~g.pre(x)~{\wedge}~\forall r \,{\cdot}\, g.post(x,r) {\implyS} f.pre(r)~{\seq}} \\
\> \> \coden{\ens~\exists r \,{\cdot}\,g.post(x,r)~{\wedge}~f.post(r,res)} 
\end{tabbing}


\noindent
where \coden{g.pre(x)} and \coden{f.pre(r)} are the pre-conditions, and
\coden{g.post(x,r)} and \coden{f.post(r,res)} are the post-conditions
for the two calls, \coden{g(x)} and \coden{f(r)} calls, respectively.
Writing such pre/post specification is considerably more complex.
Take note that this pair of pre/post specification moreover assumes
the use of pure Hoare logic. If we wish to leverage on a
more expressive separation logic; we would need to use a
different higher-order specification logic that uses existential
predicate. More specifically for this compose method, we 
may need to use the following separation logic based pre/post
specifications instead.

\begin{tabbing}
\quad \quad \= \quad \= \coden{let~r2~} \= \kill
\> \coden{compose\$(f,g,x,res)~=~\exists\, f1,f2 \,{\cdot}\,}\\
\> \> \coden{\req~g.pre(x)~{\sep}f1(x)~{\wedge}~\forall r \,{\cdot}\, g.post(x,r){\sep}f1(x)~{\entS}~f.pre(r){\sep}f2(x,r)~{\seq}} \\
\> \> \coden{\ens~\exists r \,{\cdot}\,f2(x,r)~{\sep}~f.post(r,res)} 
\end{tabbing}


\noindent
Here, \coden{\entS} denotes the entailment operator
of separation logic, while \coden{f1(x)} and \coden{f2(x,r)}
are existential predicates that need to be
computed (or provided) as anti-frame and frame conditions of
an entailment operation.
Unlike the more abstract staged specification,
pre/post specifications need to capture more details of our
underlying %
logic,
and utilize extra
higher-order unknown predicates, such as \coden{f1(x)} and \coden{f2(x,r)},
that must be suitably instantiated.

For another example of staged specification,
consider the following higher-order method which repeatedly
applies a function \coden{f} \coden{n}-times.

\begin{tabbing}
\quad \quad \= \coden{\btt{applyN}(f,x,n) =} \= if~\coden{n{==}0}~then~\coden{x} \\
\> \> else~let~\coden{r=f(x)}~in~\coden{\btt{applyN}(f,r,n{-}1)}
\end{tabbing}


As this higher-order function is recursive, pre/post specification
of such functions would typically require the use of an
{\em invariant} that holds for the pre-state for each
invocation of the function-type parameter.
This is quite similar to how loops are handled in
Hoare logic. The similarity here need not be surprising since
loops can also be implemented as a
higher-order tail-recursive function.


\begin{tabbing}
\quad \quad \= \coden{\m{applyN}\$(f,x,n,res) =} \\
\> \quad \= \req~\= \coden{(n{>}0{\ra}I(x,n)){\wedge}n{\geq}0} \\
\> \> \> \coden{\wedge~f\$(x,r)\,{=}\,\req~I(x,n){\wedge}n{>}0~\ens~I(r,n{-}1)}  \\
\> \> \ens~\coden{n{=}0{\wedge}res{=}n \vee I(res,0) {\wedge}n{>}0}
\end{tabbing}


Take note that \coden{I(x,n)} may contain heap references,
and moreover is using an \coden{n} argument that is global
to the relation \coden{f\$(x,r)}.
The main challenge in using
such pre/post specification is finding good
instantiations of \coden{I(x,n)}
for each given function-type parameter \coden{f}.


Let us now look at how we would write staged specification
for \coden{\m{applyN}}. As this method is recursive,
we need an inductive predicate
to model its specification. One possible
inductive predicate is given below with a slightly stronger pre-condition
\coden{n{\geq}0} to help ensure termination.

\begin{tabbing}
\quad \quad \= \coden{\m{applyN}\$(f,x,n,res) =} \= \coden{\req~n{=}0\,{;}~\ens~res{=}x} \\
\> \quad \quad \coden{\vee~\req~n{>}0\,{\seq}\,\exists r {\cdot} f\$(x,r)\,{\seq}\,\m{applyN}\$(f,r,n{-}1,res))} 
\end{tabbing}


The \coden{applyN} method uses
a function-type parameter
\coden{f} that could be instantiated for different
method calls. Two simple use cases
are illustrated below.

\begin{tabbing}
\quad \quad \= \coden{\btt{foo1}(x,n) =} \= \btt{applyN} (\codelam{x}{x{+}1},\coden{\,x,n}) \\
\> \coden{\btt{foo2}(x,n) =} \= \btt{applyN} (\codelam{x}{let~()=(x{:=}!x{+}1)~in~x},\coden{\,x,n})
\end{tabbing}


The first \btt{foo1} example uses
a pure integer function (\codelam{x}{x{+}1}), while
the second \btt{foo2} example uses an imperative heap-based method
(\codelam{x}{let~()=(x:=!x+1)~in~x}).
Both these lambda terms can be modelled by their
corresponding staged specifications. The first lambda
term can be modeled by its relation, namely
(\codelamB{(x,r)}{r{=}x{+}1})
with just one stage to ensure that
the result \coden{r} of the lambda function
is bound to \coden{x{+}1}.
The second lambda term requires two stages in its
specification. The first stage requires a heap
\coden{\heapto{x}{a}} to be pre-allocated, while
a second stage modifies (or updates)
its prior heap location to
\coden{\heapto{x}{r}{\wedge}r{=}a{+}1} where \coden{r}
is the result returned by the lambda function.

In both these example, we can use the
inductive \coden{\m{applyN}\$} predicate
to capture the staged specifications for
repeated execution of our lambda term,
as shown below.

\begin{tabbing}
\quad \quad \= \coden{\myit{foo1}\$(x,n,res) =} \= \coden{\m{applyN}\$((\codelamB{(x,r)}{\ens~r{=}x{+}1}),\,x,\,n,\,res)} \\
\> \coden{\myit{foo2}\$(x,n,res) =} \= \coden{\m{applyN}\$((\codelamB{(x,r)}{\req~\heapto{x}{a}~\seq~\ens~\heapto{x}{a'}{\wedge}a'{=}a{+}1{\wedge}r{=}x}),\,x,\,n,\,res)} 
\end{tabbing}


Both these use cases of inductive \coden{\m{applyN}} predicate
are concise and precise, but may be further
simplified to the following two
first-order (and non-recursive)  staged specifications:

\begin{tabbing}
\quad \quad \= \coden{\myit{foo1}\$(x,n,res) \implies} \= \coden{\req~n{\geq}0\,{\seq}\,\ens\,res{=}x+n} \\
\> \coden{\myit{foo2}\$(x,n,res) \implies} \= \coden{\req~\heapto{x}{a}{\wedge}n{\geq}0~\seq~\ens\,\heapto{x}{a'}{\wedge}a'{=}a{+}n{\wedge}res{=}x}
\end{tabbing}


A staged specification is said to be {\em first-order} if it did not
use any higher-order features, such as function-type parameters.
It is said to be {\em non-recursive} if it does not make use
of inductive predicates, such as \coden{\m{applyN}}.
These two first-order staged specifications can be confirmed
as approximation (or summarization) of the earlier
staged specifications by suitable (cyclic)
entailment proofs, namely:

\begin{tabbing}
\quad \quad \= \coden{\m{applyN}\$((\codelamB{(x,r)}{r{=}x{+}1}),\,x,\,n,\,res)} \= \entS \coden{\req~n{\geq}0\,{\seq}\,\ens\,res{=}x+n} \\
\> \coden{\m{applyN}\$((\codelamB{(x,r)}{\req~\heapto{x}{a}~\seq\,\ens\,\heapto{x}{r}{\wedge}r{=}a{+}1}),\,x,\,n,\,res)}  \\
\> \> \entS \coden{\req~\heapto{x}{a}{\wedge}n{\geq}0~\seq\,\ens\,\heapto{x}{a'}{\wedge}a'{=}a{+}n{\wedge}res{=}x} 
\end{tabbing}





















 


























  









We shall next look at more examples that can be
nimbly handled
by staged specifications.


==> entail-short.tex <==
\begin{restatable}[Soundness of entailment]{theorem}{entailsound}
\label{thm:entailsound}
Given
  $\stagesubsume{\dspec_1}{\dspec_2}$ and
  $\specbigstep{S,h}{S_1,h_1}{\dspec_1}$,
then
  there exists
  $h_2,L_2$~such that~$\specbigstep{S,h}{S_2,h_2}{\dspec_2}$ where $h_2 \subseteq h_1$.
\emph{(Here, $h_1 \subseteq h_2$ denotes that $h_1$ is a subheap of $h_2$, i.e.,~$\exi{h_3} h_1 \disjunion h_3 = h_2$.)}
\end{restatable}

\begin{proof}
  By induction on the derivation of $\stagesubsume{\dspec_1}{\dspec_2}$.
  See Appendix~\ref{sec:entail_sound}.
\end{proof}


==> impl.tex <==
\begin{verbatim}
Order (for OCaml like language)
-----
1. Parser for SLEEK tests
2. Parser for Language + Core
3. SLEEK prover
4. HIP Verifier

Experimental Evaluation
\end{verbatim}


==> intro-auto.tex <==
Automated verifiers also suffer from a different set of problems.
As they are SMT-based and cannot handle higher-order triples directly, each verifier typically resorts to implementing a bespoke theory of higher-order functions which it uses to produce first-order proof obligations.
As a result, these theories are typically restricted (to support better
automation) but are largely incompatible with each other.

Dafny does not support mutable closures\footnote{\url{https://github.com/dafny-lang/dafny/issues/3392}}.
WhyML supports higher-order functions via defunctionalization~\cite{DBLP:journals/corr/abs-2011-14044}, which is difficult to integrate with higher-order state.
Other verifiers based on the Why3 platform have language-specific assumptions (e.g.,~Rust's borrowing discipline~\cite{DBLP:conf/tacas/DenisJ23}) or aliasing restriction on references~\cite{Kanig2009WhoAV}.
Viper-based verifiers have highly varying support, as each frontend implements it in their own way~\cite{weber2017automating,milizia2022verification,DBLP:journals/pacmpl/WolffBMMS21}. Prusti~\cite{DBLP:journals/pacmpl/WolffBMMS21} is notable for having expressive set of specification constructs for higher-order behavior, but it too is specialized for the type system of Rust.
Mutable closures are not expressible in \fstar's base logic~\cite{DBLP:conf/popl/SwamyHKRDFBFSKZ16}, requiring an encoding of a new memory model for separation logic~\cite{DBLP:journals/pacmpl/SwamyRFMAM20}. The extent to which automation applies to difficult higher-order examples in this memory model is unclear~\cite[Section 6]{Fillitre2016AMW}.

In short, there is no verifier today which handles effectful higher-order functions in full generality, while being amenable to automation and affording reasonably simple, concise, precise and modular specification mechanisms.
While many uses of exceptional and mutable closures can of course be re-expressed in terms of other language features, we believe it is important to handle them, especially in verifiers tailored for existing languages, as higher-order programming can be extremely subtle and is a domain where verification helps significantly.


==> intro-old.tex <==
Higher-order programs are becoming more pervasive and
are already built natively in popular languages, such as Python and JavaScript,
and are also being incorporated into mainstream languages,
such as C\# (since 3.0) and Java (since version 8).
Higher-order features are desirable since they
allow design patterns and code reuse to be easily supported. 
However, reasoning with higher-order programs
are considerably more complex, and various programming language
researchers have been working towards better foundational mechanisms
to support their formal reasoning.
%

\citet{Contract:Findler:ICFP02} show how dynamic assertion checking system
may be used to correctly assign blames in higher-order functions.
\citet{Yoshida:FOSSACS07} show how Hoare-style pre-post logic
can be extended to support imperative higher-order functions.
Liquid Haskell \cite{Liquid:Haskell14} utilizes refinement 
types to
support data invariants and write specifications
involving higher-order functions in a purely
functional language without imperative effects.
In the work of  \citet{DanaXu:POPL09}, the authors develop
an extended static checking mechanism that can
support
precise blame assignments
in the presence of higher-order functions and laziness.

While higher-order functions can add considerable expressivity 
to programming languages, automated reasoning systems to 
support them currently have some limitations. Most of them 
are presently based
on either Hoare-style pre/post specifications or are built 
using refinements on top of dependent type systems.
Specifically, pre/post specifications currently have limited 
expressivity to support the modeling of imperative effects
and exceptions for 
unknown function-type parameters.
Pre/post specifications for each method modularly summarize 
the intentions of codes in two stages (i) expectation of 
inputs' state before the call; and (ii) enforcement of the 
program state immediately after
executing the call. However, this two-stage pre/post 
specification approach cannot be easily used in conjunction 
with unknown functions yet to be instantiated for 
function-type parameters. 

In this paper, we propose a more general specification mechanism
that allows multiple stages to be captured, including those stages
that are attributable to unbound function-type parameters.
Such a mechanism would allow us to model higher-order functions
more concisely and precisely. Moreover, each subsequent call with
instantiated higher-order arguments can be re-summarized
(without the need for code re-verification),
once their function-type parameters are known via instantiations.

As an example on the need for multiple stages,
consider a simple higher-order function \coden{goo}
with a function-type
parameter \coden{f}. This \coden{goo} method performs some imperative effects prior to
a higher-order call \coden{f(y)}, followed by more heap-based
imperative effects after the higher-order call.

\begin{tabbing}
\quad \quad \= \quad \= \coden{let~r2~} \= \kill
\> \coden{goo(f,x,y) =} \\
\> \> \coden{let~()} \> \coden{{=}~x{:=}{!}x{+}1~in} \\
\> \> \coden{let~r} \> \coden{{=}~f(y)~in} \\
\> \> \coden{let~r2} \> \coden{{=}~{!}x{+}r~in} \\
\> \> \coden{let~()} \> \coden{{=}~y{:=}r2~in} \\
\> \> \coden{r2} 
\end{tabbing}




Writing specifications for such higher-order functions is non-trivial 
using just pre/post specifications since we have to consider unknown 
higher-order function calls, e.g., \code{f}, with arbitrary effects.
Due to such a challenge, some researchers (e.g., \cite{Pottier:POPL21}) have even
resorted to imposing a restriction that only pure functions be used 
for each higher-order function that is captured under
multi-shot setting for algebraic effects,  
claiming that their approach may be unsound otherwise.
We wish to dispel such weakness with our new solution
that can model arbitrary calls to uninstantiated functions.

In this paper, we shall show that we can provide a more 
expressive way to capture specifications of higher-order functions that utilize call-by-value (strict) semantics in a sequential setting.
Our approach allows multiple stages in the method's specification. 
We refer to our new approach as {\em staged specification},
and shall highlight it via the \coden{goo} example using
a corresponding relation, aptly named as 
\coden{goo\$(\ldots,\res)} where 
the last argument \coden{\res} denotes the function's result.


{\begin{tabbing}
\quad \quad \= \quad \= \coden{\req~\heapto{x}{b} \sep \heapto{y}{\_};~\quad} \= \quad \= \kill
\> \coden{goo\$(f,x,y,\res) =} \\
\> \> \coden{\req~\heapto{x}{a};}  \> \coden{// Stage~1: requiring~x~to~be~pre\text{-}allocated} \\
\> \> \coden{\ens~\heapto{x}{a{+}1};}  \> \coden{// Stage~2: ensuring~x~is~updated} \\
\> \> \coden{\exists~r~{\cdot}~f\$(y,r);}  \> \coden{// Stage~3: spec~of~unknown~higher\text{-}order~f~call} \\
\> \> \coden{\req~\heapto{x}{b} {\sep} \heapto{y}{\_};}  \> \coden{// Stage~4: requiring~both~x, y~to~be~pre\text{-}allocated} \\
\> \> \coden{\ens~\heapto{x}{b} {\sep} \heapto{y}{\res}}  \> \coden{// Stage~5: ensuring~y~is~updated,~and~x~is~unchanged} \\
 \> \> \quad \coden{{\wedge}~ \res{=}b{+}r;} 
\end{tabbing}}


Our new specification for this \coden{goo} function 
summarizes its effects over five stages, comprising of 
two {\em require} stages (denoted by \coden{\req} keyword), 
two {\em ensure} stages (denoted by \coden{\ens} keyword)
and 
also a distinct stage for the higher-order call, e.g., 
\coden{f(y)} (denoted by a relation, namely \coden{f\$(y,r)}).
The multiple stages here are demarcated by the ubiquitous 
sequential operator \coden{\bf{;}\,}. For the heap state of 
require stages and ensure stages, we use points-to relation, 
\coden{\heapto{x}{a}}, and the spatial conjunction 
\coden{\bf{*}} from separation logic, where appropriate. 

Take note that in Stage 3, even though the higher-order 
relation \coden{f\$(y,r)} does not have direct access to 
the \coden{x} reference, it may still have indirect access via an arbitrary lambda term that can be
passed as its function-type parameter.
To model this, we currently use worst-case assumption on the 
memory footprint of each higher-order function call, which 
required a separate fresh precondition of 
\coden{\heapto{x}{b}} to be used in Stage 4
of our example specification. 
Also, each higher-order call is kept as a separate stage 
to allow us to sequence memory updates in the correct order. 
Another reason for using a separate stage for each unknown
higher-order call is to account for uncaught exceptions or 
algebraic effects that the function-type argument may invoke.
This aspect is usually ignored in existing state-of-the-art
specifications for higher-order functions. Our new solution
provide easy extensions to support exceptions and
algebraic effects.


This paper shows that staged specification is
an {\em expressive} and {\em fundamental} mechanism
for modeling higher-order programs.
It is {\em expressive} due to its conciseness, and it is
{\em fundamental} as we do not impose any restriction on
our higher-order function parameters.
Moreover, we can integrate staged specification with separation logic
in order to provide a general way for capturing heap-based
effects for higher-order functions. We refer to the resulting
combination as {\em Higher-Order Staged Separation Logic}
(abbreviated as \HSSL).
We summarize our main contributions as follows: 
\vspace{2mm}
\begin{enumerate}[leftmargin=*,labelindent=1pt]
\item \textbf{Staged Separation Logic and its Semantics:}  
Comprehensively design \HSSL\ for use by a core ML language.
 Develop the semantics of \HSSL,
capturing staged flows of heap-operations and assertions, 
explicitly revealing higher-order function invocations.


\item \textbf{Hoare-based Rules:} Targeting an ML-like language with
  both imperative effects and higher-order functions, 
we establish Hoare-based rules to modularly
capture programs' behaviors. 
Prove soundness for this new set of Hoare rules
with staged formula.


\item \textbf{The Back-end Solver for \HSSL:} 
  Design and develop a back-end solver to
  prove/disprove the entailments between two normalized \HSSL\ 
formulae.
Provide a set of normalization rules and 
entailment rules for \HSSL, and build a working implementation
for our back-end solver.

\item \textbf{Implementation and Evaluation:} 
We prototype the proposal, prove its correctness, report on experimental results, and present various 
case studies investigating \HSSL's capabilities. 

\item \textbf{Develop Inference mechanism for \HSSL:} 
  Develop additional machinery to provide partial inference of
  \HSSL~specifications for our core OCaml-based programs.
  This allows us to support a semi-automated
  approach, where users can still assist in the creative steps.
 
\end{enumerate}















==> misc.tex <==
As this higher-order function is recursive, pre/post specification
of such functions would typically require the use of an
{\em invariant} that holds for the pre-state for each
invocation of the function-type parameter.
This is quite similar to how loops are handled in
Hoare logic. The similarity here is not be surprising since
loops can also be implemented as a
higher-order tail-recursion function.


==> moreExamples.tex <==
\begin{verbatim}
let mut i = 1;
let mut j = 2; // j is captured by (mutable) reference below:
let mut cl = |x: &mut i32| -> i32 { j += *x; *x += 1; j + *x };
4
5 let r = cl(&mut i);
assert_eq!(i, 2); // the closure's side effect on its argument
7 assert_eq!(j, 3); // the closure's side effect on its captured state
8 assert_eq!(r, 5); // the closure's result

let i = ref 1
let j = ref 2
cl(x:ref int) =
  req x->a * j->b
  ens x->a+1 * j->a+b /\ res=a+b+a+1  
  req x->a /\ x=j
  ens x->2a+1 /\ res=4a+2 
 {  
   j += !x;
   x += 1;
   j + !x
  }
cl(i) // x!=j
cl(j) // x=j


let mut inc = || { x += 1; x };

let inc() =
  req x->a
  ens x->res/\res=1+1
 {
   x:=x+1;x
 }

---------------
use std::collections::HashSet;
2 let mut set = HashSet::new(); // mutable standard library set
// set->{}
3 set.insert(42); // inserts 42 into the set
// set->{42}
4 let mut cl = |i| { set.insert(i); }; // cl captures set (mutably)
// cl = \ x . ex S; req set->S;ens set->(S+{x})
5 cl(7); // (indirectly) inserts 7 into the set
// set->{42,7}
6 foo(cl); // pass cl to some higher-order function
// need to know foo has no access to "set"
// and cl is monotonically increasing?
// set->{42,7}+D
7 // (cl is no longer live here, releasing alias to set from its captured state)
8 assert!(set.contains(&42) && set.contains(&7));

set.insert(x) =
 rex S; eq set->S;ens set->(S+{x})

cl(i) =
 ex S; req set->S;ens set->(S+{x})
 {
   set.insert(i);
 }

Without knowing foo’s precise behaviour (in particular, whether/how often it calls its argument
closure), we would like to assert that both elements remain in the set. Conceptually, this is
guaranteed without needing to know anything about foo’s behaviour: the implementation of cl
only ever adds to the set, while Rust’s type system prevents there being any other usable alias to
the same set while the closure is live

 foo(f,...)
  // foo's footprint excludes set
  // f only increases set
  // hence set only increases at most

Key Problem K2: Expressing the possible evolution of a closure’s captured state across
unknown, potentially unbounded numbers of calls to the closure.

Key Problem K3: Specifying higher-order programming idioms, including suitable
requirements on closure values passed to a function.

Key Problem K4: Specifying the side effects and results of higher-order functions
parametrically in those of closure arguments they are passed.

let nums = vec![1, 2, 3];
2 let r = nums.iter() // creates an iterator over the vector
3 .map(|i| (*i) * 2)
4 .collect::<Vec<_>>(); // collects the iterator's elements into a vector
5 assert_eq!(r, vec![2, 4, 6]);

What are the specs of map and collect? How to take imperative f into
account

use std::iter::repeat_with;
2 let mut count = 0;
3 let nums = repeat_with(
4 || { let r = count; count += 1; r * 2 });
56
for i in nums.take(10) { // iterates over the first 10 values
7 assert!(i %
8 }

// how to deal with lazy + imperative evaluation?

count->0
nums.next() =
 req count->a
 ens count->a+1/\res=2a

nums_enum(nxt) = nxt():nums_enum(nxt)

nums = nums_enum(nxt)

Key Problem K5: Specifying aggregated values computed via the combination of repeated
closure calls.

let nums = vec![1, 5, 7, 11, 13];
2 let all_odd = nums.iter()
3 .fold(true, |a, c| a && (c %
45
if all_odd {
6 for i in nums {
7 assert!(i %
8 }
9 }

Key Problem K6: Relating closure behaviour to abstract mathematical relations and
predicates.

K1 : Closure Property

let mut a = 0;
// a->0
2 let mut cl =
3 #[requires(true)]
4 #[ensures(a == old(a) + i && result == a)]
5 |i: i32| { a += i; a }; // captures a by mutable reference
// a->0/\cl=\i r-> ex x; req a->x; ens a->res/\res=x+i
// closure(a,0,cl)
6 assert_eq!(cl(1), 1); // 
// closure(a,1,cl)
7 assert_eq!(cl(2), 3);
// closure(a,3,cl)

cl(i) 
  req a->x
  ens a->res/\res=x+i
  = {
      a+=i; a
    }

closures are pure function values
where Prusti effectively represent it as a closure pred.
  closure(a,y,f) = a->y /\ f=\i r . req a->x;ens a->res/\res=x+1
    /\ y>=0

Heifer solution?
 cl::closure(a,y,f)
 // it has some state and a function f

let mut count = 0;
2 let mut cl =
3 #[invariant(count >= 0)]
4 #[ensures(count == old(count) + 1 && result == count)]
5 #[ensures(result > 0)]
6 || { count += 1; count };

  //cl::closure(a,y,f)
let i = cl();
  //cl::closure(a,y+1,f)
2 foo(&mut cl);
  //cl::closure(a,z,f)/\z>=y+1
3 let j = cl();
  //cl::closure(a,z+1,f)/\z>=y+1
4 assert!(i < j);

For this purpose, we introduce specification entailments, assertions of the form
cl |= |a1, a2, . . . | { requires Pexp, ensures Qexp } ,
#[ensures(result > 0)]
2 fn roll_dice() -> i32 { /* ... */ }
34
#[requires(f |= |i: i32| { requires(i > 0), ensures(result > 0) })]
5 #[ensures(result > 0)]
6 fn call_ret(mut f: impl FnMut (i32) -> i32) -> i32 {
7  let x = roll_dice();
8  return f(x);
9 }

Heifer:
 call_ret(f,res)
  = ens x>0;f(x,r);ens res=r

Prusti-1 (pg 11, Fig 3)
 req f <: \(i,res). req i>0 ens res>0
 ens res>0

Prusti-2 (pg 13, Fig 3)
 req f <: \(i,res). req i>0 ens true
 ens ex i: i>0 && old(f)(i) ~~> {result==outer(result)}

// poor man sequencing?


let cl =
2 #[requires(i > 0)]
3 #[ensures(result > 42 && result %
4 |i: i32| -> i32 { 42 + 2 * i };
5 let r = call_ret(cl);
6 assert!(r > 42 && r %


roll_dice(res) = res>0

call_ret(f,res) =
 req f <: \(i,res). req i>0 ens res>0
 ens res>0
{
}

let mut x = -1;
2 let mut cl =
3 #[invariant(x >= old(x))] // shouldn't it be x>old(x)
4 #[requires(i > 0)]
5 #[ensures(result == old(x) && x == old(x) + i)]
6 |i: i32| { let r = x; x += i; r };
7 // L1
8 cl(2);
9 // L2
10 call_ret(cl);

We therefore introduce a specialized single-call specification entailment
|=!, expressing that the closure instance on its left-hand side fulfills the expected specification for
its next call.

invariant + history invariant
single-cal spec entailment

Key Problem K1: How to specify guaranteed closure behaviour for all future call sites,
potentially conditioned on values of the closure’s captured state.

Key Problem K2: Expressing the possible evolution of a closure’s captured state across
unknown, potentially unbounded numbers of calls to the closure.

Key Problem K3: Specifying higher-order programming idioms, including suitable
requirements on closure values passed to a function.

Key Problem K4: Specifying the side effects and results of higher-order functions
parametrically in those of closure arguments they are passed.

Key Problem K5: Specifying aggregated values computed via the combination of repeated
closure calls.

Key Problem K6: Relating closure behaviour to abstract mathematical relations and
predicates.

#[ghost_arg(inv: Fn(&Vec<T>, usize, A) -> bool)]
2 #[requires(inv(v, 0, init))]
3 #[requires(forall n: usize ::
4 n < v.len() ==>
5 f |= |a, c| { requires(inv(outer(v), outer(n), a)
6 && outer(v[n]) == c),
7 ensures(inv(outer(v), outer(n) + 1, result)) } )]
8 #[ensures(inv(v, v.len(), result))]
9 fn fold_vec<T, A> (v: &Vec<T>, init: A, mut f: impl FnMut (A, &T) -> A)
10 -> A {
11 let mut acc = init;
12 for el in v {
13 acc = f (acc, el);
14 }
15 acc
16 }

ex P, Inv;
req List(l,xs) * Inv([],a) /\ all(P,xs) /\
     f<:\(x,a',r).ex ys; req Inv(ys,a')/\P(x) -> Inv(x:ys,r)
ens List(l,xs) * Inv(xs,res)
\end{verbatim}



==> presentation.tex <==

\newpage

$\varphi = \stagereq{\heap{\wedge}\pure} \mid \stageens{\heap{\wedge}\pure} \mid \varphi \seq \varphi \mid f(x, r) \mid \stageexi{y}\varphi \mid \varphi\vee\varphi$

\bigskip

$\begin{array}{r@{\hspace{0.5em}}c@{\hspace{0.5em}}l@{\hspace{0.7em}}l}
\s{P}\ e\ \s{Q} & \equiv & \forall \sigma, \sigma' \cdot \langle \sigma, e \rangle \longrightarrow \langle \sigma', v \rangle, & P\ \sigma \implies Q\ v\ \sigma' \\
&&& \\
\s{\stageens{\emp}}\ e\ \s{\varphi} & \equiv & \forall \sigma, \sigma' \cdot \langle \sigma, e \rangle \longrightarrow \langle \sigma', v \rangle, & \langle \sigma \leadsto \sigma', v \rangle \vDash \varphi
\end{array}$

\bigskip

\begin{lstlisting}[name=foldrr]
let count = ref 0 in
foldr (fun c t -> incr count; c + t) 0 xs
\end{lstlisting}

\begin{lstlisting}[name=composeeee]
let compose f g x = f (g x)
\end{lstlisting}



{\small 
\begin{tabbing}
  \  \= \quad \= \coden{\req~\heapto{x}{b} \sep \heapto{y}{\_};~\quad\quad\quad\quad\quad} \= \quad \= \kill
\> \coden{\stageho{hello}{f,x,y,\res} =} \\
\> \> \coden{\stageexi{a}\stagereq{\heapto{x}{a}}\seq\stageens{\heapto{x}{a{+}1}}\seq}  \> \\
\> \> \coden{\stageexi{r}\stageho{f}{y,r}\seq}  \>  \\
\> \> \coden{\stageexi{b}~\stagereq{\heapto{x}{b}} {\sep} \heapto{y}{\_};}  \>  \\
\> \> \phantom{\coden{\stageexi{b}~}}\coden{\stageens{\heapto{x}{b}} {\sep} \heapto{y}{\res}{\wedge}\res{=}b{+}r}  \> 
\end{tabbing}}

\begin{lstlisting}[name=helloo]
let z = ref 0 in
hello (fun _ -> incr z; 0) z (ref 1)
\end{lstlisting}

$f(y, \res) = \stageexi{c}\stagereq{\heapto{x}{c}\seq\stageens{\heapto{x}{c{+}1}{\wedge}\res{=}0}}$

\bigskip

$compose(f, g, x, \res) = \stageexi{r}\stageho{g}{x, r}\seq\stageho{f}{r,\res}$

{\small 
\begin{tabbing}
  \  \= \quad \= \coden{\req~\heapto{x}{b} \sep \heapto{y}{\_};~\quad\quad\quad\quad\quad} \= \quad \= \kill
\> \coden{\stageho{hello}{f,x,y,\res} =} \\
\> \> \coden{\stageexi{a}\stagereq{\heapto{x}{a}}\seq\stageens{\heapto{x}{a{+}1}}\seq}  \> \\
\> \> \coden{\stageexi{r, c}\stagereq{\heapto{x}{c}}\seq\stageens{\heapto{x}{c{+}1}{\wedge}r{=}0}}  \>  \\
\> \> \coden{\stageexi{b}~\stagereq{\heapto{x}{b}} {\sep} \heapto{y}{\_};}  \>  \\
\> \> \phantom{\coden{\stageexi{b}~}}\coden{\stageens{\heapto{x}{b}} {\sep} \heapto{y}{\res}{\wedge}\res{=}b{+}r}  \> 
\end{tabbing}}

$\seplogicentail{\heapto{x}{a{+}1}\sep (a{+}1{=}c)}{\heapto{x}{c}\sep\emp}$

{\small 
\begin{tabbing}
  \  \= \quad \= \coden{\req~\heapto{x}{b} \sep \heapto{y}{\_};~\quad\quad\quad\quad\quad} \= \quad \= \kill
\> \coden{\stageho{hello}{f,x,y,\res} =} \\
\> \> \coden{\stageexi{a}\stagereq{\heapto{x}{a}}\seq\stageexi{c}\stagereq{a{+}1{=}c}\seq}  \> \\
\> \> \coden{\stageexi{r}\stageens{\emp}\seq\stageens{\heapto{x}{c{+}1}{\wedge}r{=}0}\seq}  \>  \\
\> \> \coden{\stageexi{b}~\stagereq{\heapto{x}{b}} {\sep} \heapto{y}{\_};}  \>  \\
\> \> \phantom{\coden{\stageexi{b}~}}\coden{\stageens{\heapto{x}{b}} {\sep} \heapto{y}{\res}{\wedge}\res{=}b{+}r}  \> 
\end{tabbing}}

{\small 
\begin{tabbing}
  \  \= \quad \= \coden{\req~\heapto{x}{b} \sep \heapto{y}{\_};~\quad\quad\quad\quad\quad} \= \quad \= \kill
\> \coden{\stageho{hello}{f,x,y,\res} =} \\
\> \> \coden{\stageexi{a,c}\stagereq{\heapto{x}{a}{\wedge}a{+}1{=}c}\seq}  \> \\
\> \> \coden{\stageexi{r}\stageens{\heapto{x}{c{+}1}{\wedge}r{=}0}\seq}  \>  \\
\> \> \coden{\stageexi{b}~\stagereq{\heapto{x}{b}} {\sep} \heapto{y}{\_};}  \>  \\
\> \> \phantom{\coden{\stageexi{b}~}}\coden{\stageens{\heapto{x}{b}} {\sep} \heapto{y}{\res}{\wedge}\res{=}b{+}r}  \> 
\end{tabbing}}

$\seplogicentail{\heapto{x}{c{+}1{\wedge}r{=}0}\sep (c{+}1{=}b{\wedge}\heapto{y}{\_})}{\heapto{x}{b}{\sep}\heapto{y}{\_}\sep r{=}0}$

{\small 
\begin{tabbing}
  \  \= \quad \= \coden{\req~\heapto{x}{b} \sep \heapto{y}{\_};~\quad\quad\quad\quad\quad} \= \quad \= \kill
\> \coden{\stageho{hello}{f,x,y,\res} =} \\
\> \> \coden{\stageexi{a,c}\stagereq{\heapto{x}{a}{\wedge}a{+}1{=}c}\seq}  \> \\
\> \> \coden{\stageexi{r}\stagereq{c{+}1{=}b{\wedge}\heapto{y}{\_}}\seq}  \>  \\
\> \> \coden{\stageexi{b}~\stageens{r{=}0}}\seq  \>  \\
\> \> \phantom{\coden{\stageexi{b}~}}\coden{\stageens{\heapto{x}{b}} {\sep} \heapto{y}{\res}{\wedge}\res{=}b{+}r}  \> 
\end{tabbing}}

{\small 
\begin{tabbing}
  \  \= \quad \= \coden{\req~\heapto{x}{b} \sep \heapto{y}{\_};~\quad\quad\quad\quad\quad} \= \quad \= \kill
\> \coden{\stageho{hello}{f,x,y,\res} =} \\
\> \> \coden{\stageexi{a,c,r}\stagereq{\heapto{x}{a}{\sep}\heapto{y}{\_}\wedge c{+}1{=}b{\wedge}a{+}1{=}c}\seq}  \> \\
\> \> \coden{\stageexi{b}~\stageens{\heapto{x}{b}{\sep}\heapto{y}{\res}\wedge r{=}0{\wedge}\res{=}b{+}r}}\seq  \>  \\
\end{tabbing}}

{\small 
\begin{tabbing}
  \  \= \quad \= \coden{\req~\heapto{x}{b} \sep \heapto{y}{\_};~\quad\quad\quad\quad\quad} \= \quad \= \kill
\> \coden{\stageho{hello}{f,x,y,\res} =} \\
\> \> \coden{\stageexi{a}\stagereq{\heapto{x}{a}{\sep}\heapto{y}{\_}}\seq}  \> \\
\> \> \coden{\stageens{\heapto{x}{a{+}2}{\sep}\heapto{y}{\res}\wedge\res{=}a{+}2}}\seq  \>  \\
\end{tabbing}}


\[
  \fai{x,n,\res}\stageho{applyN}{incr,x,n,\res}
  \stagesubs
  \stagereq{n{\geq}0}~\stageens{\res{=}x{+}n}
\]


{\tiny %
  \[\inferrule*[Right=Unfold]
  {\inferrule*[Right=Rewrite]
  {\inferrule*[Right=Unfold]
  {\inferrule*[Right=Normalize]
  {\inferrule*[Right=EntNorm]
  {n \geq 0 \implies \m{true} \\ \res=(x+1)+n-1 \implies \res=x+n }
  {\fbox{\stageens{n > 0 \wedge r=x+1 \wedge \res=r+n-1}} \stagesubs \stagereq{n\geq 0}\seq\stageens{\res=x+n}}}
  {\stageens{n {>} 0}\seq\fbox{(\stageens{r{=}x{+}1})}\seq(\stagereq{n{-}1\geq 0}\seq\stageens{\res{=}x{+}n{-}1}) \stagesubs \stagereq{n{\geq} 0}\seq\stageens{\res{=}x{+}n}}}
  {\stageens{n {>} 0}\seq\stageho{inc}{x, r}\seq\fbox{(\stagereq{n{-}1\geq 0}\seq\stageens{\res{=}x{+}n{-}1})} \stagesubs \stagereq{n{\geq} 0}\seq\stageens{\res{=}x{+}n}}}
  {\fbox{(... $\vee$ \stageens{n > 0}\seq\stageho{inc}{x, r}\seq\stageho{\m{applyN}}{inc, n-1, r, \res})} \stagesubs \stagereq{n\geq 0}\seq\stageens{\res=x+n}}}
    {\stageho{\m{applyN}}{inc, n, x, \res} \stagesubs \stagereq{n\geq 0}\seq\stageens{res=x+n}}
\qquad\quad 
\]}

{\small %
  \[\inferrule*[Right=Unfold]
  {\inferrule*[Right=Rewrite]
  {\inferrule*[Right=Unfold]
  {\inferrule*[Right=Normalize]
  {\inferrule*[Right=EntNorm]
  {\inferrule*[Right=SMT]
  { \phantom{a} }
  {\m{xs}{=}h{::}t{\wedge}\res{=}h{+}\m{sum}(t){+}k \implies \res{=}\m{sum}(\m{xs}){+}k}}
  {\stageexi{h,t}\stageens{\m{xs}{=}h{::}t{\wedge}\res{=}h{+}\m{sum}(t){+}k} \stagesubs
  \stageens{\res{=}\m{sum}(\m{xs}){+}k}}}
  {\stageexi{r_1,h,t}\stageens{\m{xs}{=}h{::}t}\seq\stageens{r_1=\m{sum}(t){+}k}\seq\stageens{\res{=}h{+}r_1} \stagesubs \stageens{\res{=}\m{sum}(\m{xs}){+}k}}}
  {\stageexi{r_1,h,t}\stageens{\m{xs}{=}h{::}t}\seq\stageens{r_1{=}\m{sum}(t){+}k}\seq\stageho{\m{plus}}{h,r_1,\res} \stagesubs \stageens{\res{=}\m{sum}(\m{xs}){+}k}}}
  {(... \vee \stageexi{r_1,h,t}\stageens{\m{xs}{=}h{::}t}\seq\stageho{\m{foldr}}{\m{plus},t,k,r_1}\seq\stageho{\m{plus}}{h,r_1,\res}) \stagesubs \stageens{\res{=}\m{sum}(\m{xs})+k}}}
    {\forall \m{xs},k,\res\cdot\stageho{\m{foldr}}{\m{plus}, \m{xs}, k, \res} \stagesubs \stageens{\res{=}\m{sum}(\m{xs}){+}k}}
\qquad\quad 
\]}




